Robust PCA for Subspace Estimation in User-Centric Cell-Free Wireless Networks

We consider a scalable user-centric cell-free massive MIMO network with distributed remote radio units (RUs), enabling macrodiversity and joint processing. Due to the limited uplink (UL) pilot dimension, multiuser interference in the UL pilot transmission phase makes channel estimation a non-trivial problem. We make use of two types of UL pilot signals, sounding reference signal (SRS) and demodulation reference signal (DMRS) pilots, for the estimation of the channel subspace and its instantaneous realization, respectively. The SRS pilots are transmitted over multiple time slots and resource blocks according to a Latin squares based hopping scheme, which aims at averaging out the interference of different SRS co-pilot users. We propose a robust principle component analysis approach for channel subspace estimation from the SRS signal samples, employed at the RUs for each associated user. The estimated subspace is further used at the RUs for DMRS pilot decontamination and instantaneous channel estimation. We provide numerical simulations to compare the system performance using our subspace and channel estimation scheme with the cases of ideal partial subspace/channel knowledge and pilot matching channel estimation. The results show that a system with a properly designed SRS pilot hopping scheme can closely approximate the performance of a genie-aided system.

==> 01b_introduction.tex <==
%!TEX root = isit-paper.tex

\section{Introduction} 

Consider a scalable user-centric cell-free wireless network with $L$ remote radio heads (RRHs), each with $M$ antennas, and $K$ single-antennas user equipments (UEs), where finite size clusters of RRHs are connected to each UE.
We study the uplink (UL) pilot and data transmission, and use the received sounding reference signal (SRS) and demodulation reference signal (DMRS) pilots at the RRHs for the estimation of the channel subspace and realization \cite{3gpp38211}. Thanks to TDD operations and channel reciprocity, these estimates could also be used for the downlink \cite{marzetta2010noncooperative}. We note that, compared to the channel realization, the channel subspace changes on a much larger time scale and is constant over multiple resource blocks, and thus separate the assignment of SRS and DMRS pilots, maintaining the same RRH clusters associated to the UEs. Although many works investigating cell-free wireless networks assume channel covariance matrices to be known throughout the system or at the RRHs serving a UE (see \cite{9336188} for an overview), this knowledge is not easy to obtain in practical systems. Additionally, obtaining the channel subspace information is less demanding and more robust.
We focus in this paper on an SRS pilot assignment scheme aiming at reducing pilot contamination and a subspace estimation approach, such that the estimated subspace is used in place of the covariance matrix for further signal processing.

Subspace estimation based on Approximate Maximum-Likelihood (AML) is proposed in \cite{8264736} for a massive MIMO system, where the basic estimation problem for a single user without multiuser interference is studied.
Principle Component Analysis (PCA) for subspace estimation in a massive MIMO system is employed in \cite{9136836}, under the assumptions that no inter-cell interference occurs and that the BS receives signals from all users on the same multipaths. The estimated direction of arrival angles are thus the same for all users in the cell and only the channel gains are estimated per user with UL pilots.
In case of multiuser interference from different multipaths however, the received signals over time at the BS used for subspace estimation contain the UL signal from various users and possibly outliers, i.e., samples whose dominant subspace differs from the subspace of the desired signal. A PCA approach for datasets corrupted with outliers might lead to inaccurate estimates, which motivates the employment of {\em robust} PCA (R-PCA) that is able to identify these outliers and to find the underlying low-dimensional subspace of the inliers. We refer to \cite{8425657} for an overview of different robust PCA approaches.

In this work, we consider a cell-free wireless network, where all $K$ users send a sequence of $\tausrs < K$ orthogonal sounding reference signal (SRS) pilots in the UL, yielding SRS pilot contamination and thus possibly outliers. We develop an SRS pilot sequence assignment based on latin squares \cite{467960} such that the geographic distance of co-pilot users is large, and propose the R-PCA algorithm from \cite{6126034} at the RRHs for subspace estimation of their associated users. We show that the two proposed schemes lead to accurate subspace estimates being able to closely approach the system performance of the genie-aided cases of perfect subspace knowledge and ideal channel state information, respectively.

%{\em Multiuser MIMO} is a key transformative technology at the center of the last decade of theoretical research and 
%practical system design, since the first information theoretical break through of
%Caire and Shamai \cite{caire2003achievable}, to the provisions in recent wireless standards \cite{3gpp38211}. 
%A successful related concept is Marzetta's {\em massive MIMO} \cite{marzetta2010noncooperative}. 
%This is based on the observation that, thanks to channel reciprocity and TDD operations,  
%an arbitrarily large number $M$ of base station (BS) antennas can be trained by a finite number $K$ of user equipments (UE) 
%using a finite-dimensional uplink (UL) pilot field $\tau_p \geq K$. 
%Since the channel coherence block of $T$ channel uses\footnote{We define a channel coherence block as a ``tile'' of $T$ symbols in the time-frequency domain over which the fading channel can be considered constant. For the sake of conceptual simplicity, this can be identified as resource block (RB) 
%of the underlying PHY protocol.}  is limited by the channel time and frequency selectivity, in a large cellular network the number of  simultaneoutly active users $K$ is generally much larger than $\tau_p$. This implies that mutually non-orthogonal pilot sequences are used in different cells 
%yielding  {\em pilot contamination}, which creates a coherently combined term in the
%inter-cell interference that does not vanish as $M \rightarrow \infty$ \cite{marzetta2010noncooperative}.  
%More recently, a flurry of works advocating the joint processing of spatially distributed remote radio heads (RRHs) has appeared. 
%This idea can be traced back to the work of Wyner \cite{wyner1994shannon}, and has been ``re-marketed''  several times under different names with slight nuances, 
%such as {\em coordinate multipoint} (CoMP),  {\em cloud radio access network} (CRAN), or {\em cell-free massive MIMO}. 
%An excellent recent review of this vast literature is given in \cite{9336188}. While these approaches were initially marketed as 
%``eliminating inter-cell interference'',  this is unfortunately not quite true since the pilot contamination problem due to the limited UL pilot dimension persists even with full joint processing of all the RRHs. In addition, other challenges emerge. 
%First, deploying a number of RRHs much larger than the number of UEs is often infeasible, especially for outdoor systems.  
%Second, the joint processing of all RRHs across the network  yield a non-scalable architecture. 
%
%In this work, we consider the realistic case of a network covering an area $A$, where the number of RRHs $L$ is less than the number of users $K$ simultaneously 
%active on any given resource block (RB). However, we allow each RRH to have an $M$-antennas array, such that the total number of antenna elements $ML$ is generally larger than $K$.  We employ a scalable {\em user-centric} architecture based on dynamic cluster formation, as proposed in several recent papers
%(see \cite{9336188}), such that every UE is served by a finite-size cluster of RRHs even  if the network is arbitrarily large. 
%We extend our previous work \cite{goettsch2021impact} by investigating DL precoding and power allocation schemes. 
%UL-DL SINR duality in cell-free wireless networks was studied in \cite{9064545} and shown to hold in terms of the Signal to Interference plus Noise (SINR) 
%expression resulting from the so-called {\em use-and-then-forget (UatF) bound}, where all necessary terms to compute the ``true'' UatF bound are assumed 
%to be somehow known to a central processor devoted to DL power allocation. 
%Unfortunately, the UatF bound yields often overly pessimistic results in terms of achievable rate especially in the context of cell-free networks where the channel hardening phenomenon is not as pronounced as in standard cellular massive MIMO networks. Therefore, in this paper we consider the so-called ``optimistic ergodic rate'', i.e., the achievable rate when the UE receiver knows the useful signal term and and the interference plus noise power. 
%
%We show a new UL-DL duality in terms of SINR expressions that are actually computable by the central processor using the knowledge of the large
%scale fading coefficients (LSFC) and the {\em partial} CSI available at the RRHs through the cluster formation and UL pilot allocation. 
%Although these SINR expressions, referred to as ``nominal SINR'' in this work, do not correspond to any achievable rate, we show  via extensive simulation that 
%the UL and DL optimistic ergodic rates when the DL power is allocated through this form of duality are virtually identical. 
%This ``nominal duality''  has the advantage that no DL precoding vectors need to be computed, as they are defined to be equal to the UL combing vectors. However, 
%it incurs the disadvantage of centralized power allocation computation, requiring $O(K^2)$ signal coefficients to be collected at a processing unit to compute 
%the duality DL powers.  We compare the DL rates achieved with the proposed nominal UL-DL duality to equal power allocation (EPA) 
%and a fully distributed scheme from \cite{9069486} adapted to a system with user-centric clusters. 





















==> 02_system.tex <==
%!TEX root = isit-paper.tex
\section{System model}
We consider a cell-free wireless network in TDD operation with $L$ RRHs, each with $M$ antennas, and $K$ UEs. The set $\Cc_k \subseteq [L] = \{1,2,\dots, L\}$ denotes the cluster of RRHs serving UE $k$ and the set $\Uc_\ell \subseteq [K]$ the cluster of UEs connected to RRH $\ell$, where the cluster formation and DMRS pilot assignment for channel estimation follow the schemes in \cite{goettsch2021impact}. The RRH-UE associations are described by a bipartite graph $\Gc$ whose vertices are the RRHs and UEs, respectively. The set of edges accounting for associated RRH-UE pairs is denoted by $\Ec$, i.e., $\Gc = \Gc([L], [K], \Ec)$. We consider OFDM modulation and channels following the standard block-fading model \cite{marzetta2010noncooperative,9336188,9064545}, such that they are random but constant over coherence blocks of $T$ signal dimensions in the time-frequency domain. 

We denote by $\HH \in \CC^{LM \times K}$ the channel matrix between all $LM$ RRH antennas and all $K$ UE antennas on a given RB, where the $M \times 1$ block $\hv_{\ell,k}$ in the position corresponding to RRH $\ell$ and UE $k$ denotes the channel between this RRH-UE pair. We consider the {\em ideal partial CSI} regime, where each RRH has perfect channel knowledge for its associated UEs. The known channel matrix of a cluster $\Cc_k$ is denoted by $\HH(\Cc_k) \in \CC^{LM \times K}$,
whose $M \times 1$ blocks of RRH-UE pairs $(\ell,j) \in \Ec$ with $\ell \in \Cc_k$ are equal to $\hv_{\ell,j}$, and equal to $\zerov$ otherwise. 
The indiviudal channels between RRHs and UEs follow the simplified single ring local scattering model \cite{adhikary2013joint}, and $\Fm$ denotes the $M \times M$ unitary DFT matrix with $(m,n)$-elements
$\Fm_{m,n} = \frac{e^{-j\frac{2\pi}{M} mn}}{\sqrt{M}}$ for  $m, n  = 0,1,\ldots, M-1$.
Then, the channel between RRH $\ell$ and UE $k$ is
\begin{equation} 
	\hv_{\ell,k} = \sqrt{\frac{\beta_{\ell,k} M}{|\Sc_{\ell,k}|}}  \Fm_{\ell,k} \nuv_{\ell, k},
\end{equation}
where $\Sc_{\ell,k} \subseteq \{0,\ldots, M-1\}$, $\nuv_{\ell,k}$ and $\beta_{\ell,k}$ are the angular support set according to \cite{adhikary2013joint}, an $|\Sc_{\ell,k}| \times 1$ i.i.d. Gaussian vector with components 
$\sim \Cc\Nc(0,1)$, and the LSFC including
pathloss, blocking effects and shadowing, respectively. 
Using a Matlab-like notation, $\Fm_{\ell,k} \eqdef \Fm(: , \Sc_{\ell,k})$ denotes the tall unitary matrix obtained by selecting the columns of $\Fm$ corresponding to the index set $\Sc_{\ell,k}$.











%%We refer the reader to our previous work \cite{goettsch2021impact} for a detailed system model description, and provide a summary in the following. We consider a cell-free wireless network in TDD operation mode with $L$ RRHs, each equipped with $M$ antennas, 
%%and $K$ single-antenna UEs. Both RRHs and UEs are distributed on a squared region on the 2-dimensional plane. 
%%As a result of the cluster formation process specified in \cite{goettsch2021impact} with SNR threshold $\eta$, each UE $k$ is associated with a cluster $\Cc_k \subseteq [L] = \{1,2,\dots,L\}$ of RRHs 
%%and each RRH $\ell$ has a set of associated UEs $\Uc_\ell \subseteq [K]$. 
%The UE-RRH association is described by 
%a bipartite graph $\Gc$ with two classes of nodes (UEs and RRHs) such that the neighborhood of UE-node $k$ is $\Cc_k$ 
%and the neighborhood of RRH-node $\ell$ is $\Uc_\ell$. The set of edges of $\Gc$ is denoted by $\Ec$, i.e., $\Gc = \Gc([L], [K], \Ec)$. 
%We assume OFDM modulation and that the channel in the time-frequency domain follows the
%standard block-fading model \cite{marzetta2010noncooperative,9336188,9064545}. The channel vectors from UEs to RRHs are random but constant over coherence blocks of 
%$T$ signal dimensions in the time-frequency domain.
%%%, where $N_{\rm rb}$ and $N_{\rm sub}$ indicate  the number of OFDM symbols in time and the number of OFDM subcarriers in frequency forming a RB. 
%%%, and these quantities are chosen such that 
%%%the resource block time duration and frequency width are significantly smaller than the channel coherence time and coherence 
%%%bandwidth, respectively. 
%%The described methods are formulated for one RB, so the RB index is omitted for simplicity. 
%
%We denote by $\HH \in \CC^{LM \times K}$ the channel matrix between all the $K$ UE antennas and all the $LM$ 
%RRH antennas on a given RB, formed by $M \times 1$ blocks $\hv_{\ell,k}$ in correspondence of the $M$ antennas of RRH $\ell$ 
%and UE $k$. 
%%, i.e.,  
%%the only known channel vectors (up to estimation noise) are the vectors $\hv_{\ell,k}$ such that $(\ell,k) \in \Ec$. 
%%Hence, each RRH has a partial (noisy) view of the matrix $\HH$.  
%We define the {\em ideal partial CSI} regime,
%where each RRH $\ell$ has perfect knowledge of the channel vectors $\hv_{\ell,k}$ for $k \in \Uc_\ell$. 
%In this regime, the part of the channel matrix $\HH$ known  at the decentralized processing unit serving cluster $\Cc_k$ 
%is denoted by $\HH(\Cc_k)$. This matrix has the same dimensions as $\HH$,  such that the $(\ell, j)$ block 
%of dimension $M \times 1$  of $\HH(\Cc_k)$ is equal to $\hv_{\ell,j}$ for all  $(\ell, j) \in \Ec$, where $\ell \in \Cc_k$, and to $\zerov$ otherwise.  
%Let $\Fm$ denote the $M \times M$ unitary DFT matrix with $(m,n)$-elements
%$\Fm_{m,n} = \frac{e^{-j\frac{2\pi}{M} mn}}{\sqrt{M}}$ for  $m, n  = 0,1,\ldots, M-1$, and consider the angular support set $\Sc_{\ell,k} \subseteq \{0,\ldots, M-1\}$ 
%obtained according to the single ring local scattering model (see \cite{adhikary2013joint}). Then, the channel between RRH $\ell$ and UE $k$ is
%\begin{equation} 
%	\hv_{\ell,k} = \sqrt{\frac{\beta_{\ell,k} M}{|\Sc_{\ell,k}|}}  \Fm_{\ell,k} \nuv_{\ell, k},
%\end{equation}
%where, using a Matlab-like notation, $\Fm_{\ell,k} \eqdef \Fm(: , \Sc_{\ell,k})$ denotes the tall unitary matrix obtained by selecting the columns 
%of $\Fm$ corresponding to the index set $\Sc_{\ell,k}$, $\beta_{\ell,k}$ is the LSFC including
%pathloss, blocking effects, and shadowing, and  $\nuv_{\ell,k}$ is an $|\Sc_{\ell,k}| \times 1$ i.i.d. Gaussian vector with components 
%$\sim \Cc\Nc(0,1)$. 

\subsection{Uplink data transmission} 
The UEs transmit with the same power $P^{\rm ue}$,  and we define the system parameter $\SNR \eqdef P^{\rm ue}/N_0$, 
where $N_0$ denotes the noise power spectral density.
The received $LM \times 1$ symbol vector at the $LM$ RRH antennas for a single channel use of the UL is given by
\begin{equation} 
	\yy^{\rm ul} = \sqrt{\SNR} \; \HH \sss^{\rm ul}   + \zz^{\rm ul}, \label{ULchannel}
\end{equation}
where $\sss^{\rm ul} \in \CC^{K \times 1}$ is the vector
of information symbols transmitted by the UEs (zero-mean unit variance and mutually independent random variables) and 
$\zz^{\rm ul}$ is an i.i.d. noise vector with components $\sim \Cc\Nc(0,1)$.  
The goal of cluster $\Cc_k$ is to produce an effective channel observation for symbol $s^{\rm ul}_k$ 
(the $k$-th component of the vector $\sss^{\rm ul}$ from the collectively received signal at the RRHs $\ell \in \Cc_k$).  
We  define the receiver {\em unit norm} vector $\vvv_k \in \CC^{LM \times 1}$ formed by $M \times 1$ blocks
$\vv_{\ell,k} : \ell = 1, \ldots, L$, such that $\vv_{\ell,k} = \zerov$ (the identically zero vector) if $(\ell,k) \notin \Ec$. 
This reflects the fact that only the RRHs in $\Cc_k$ are involved in producing a received observation for the detection of user $k$. 
The non-zero blocks $\vv_{\ell,k} :  \ell \in \Cc_k$ contain the receiver combining vectors.
The corresponding scalar combined observation for symbol $s^{\rm ul}_k$ is given by 
\begin{eqnarray}
	r^{\rm ul}_k  & = & \vvv_k^\herm \yy^{\rm ul}. 
%	& = & \sqrt{\SNR} \vvv_k^\herm \hh_k s^{\rm ul}_k   + \sqrt{\SNR} \vvv_k^\herm \HH_k \sss_k^{\rm ul}  + \vvv_k^\herm \zz^{\rm ul}
\end{eqnarray}
%
%
%where $\hh_k$ denotes the $k$-th column of $\HH$, 
%$\HH_k$ is obtained by deleting the $k$-th column from $\HH$, 
%and $\sss_k^{\rm ul} $ is the vector $\sss^{\rm ul}$ after deletion of the $k$-th element. 
%
For simplicity, we assume that the channel decoder has perfect knowledge of the exact UL signal to Interference plus noise ratio (SINR) value 
\begin{eqnarray} 
	\SINR^{\rm ul}_k 
%	& = & \frac{\SNR |\vvv_k^\herm \hh_k|^2}{ \vvv_k^\herm \left ( \Id + \SNR \; \HH_k \HH_k^\herm \right ) \vvv_k} \\
& = & \frac{  |\vvv_k^\herm \hh_k|^2 }{ \SNR^{-1}  + \sum_{j \neq k} |\vvv_k^\herm \hh_j |^2 },  \label{UL-SINR-unitnorm}
\end{eqnarray}
where $\hh_k$ denotes the $k$-th column of $\HH$. The corresponding UL {\em optimistic ergodic} achievable rate is given by 
\begin{equation}
R_k^{\rm ul} = \EE [ \log ( 1 + \SINR^{\rm ul}_k ) ], \label{ergodic-rate}
\end{equation}
where the expectation is with respect to the small scale fading, while conditioning on the placement of UEs and RRH, and on the cluster formation. 

%\subsection{Downlink data transmission} 
%The signal corresponding to one channel use of the DL at the receiver of UE $k$ is given by 
%\begin{equation} 
%	y_k^{\rm dl} = \hh_k^\herm \xx  + z_k^{\rm dl},  \label{DLchannel}
%\end{equation}
%where the transmitted vector $\xx \in \CC^{LM \times 1}$ is formed by all the signal samples sent collectively from the RRHs. Without loss of generality
%we can incorporate a common factor ${\SNR}^{-1/2}$ in the LSFCs, which is equivalent to rescaling the noise at the UEs receivers such that  
%$z_k^{\rm dl} \sim \Cc\Nc(0, \SNR^{-1})$, while keeping $\beta_{\ell,k}$ for all $(\ell,k)$ identical to the UL case.
%Let $\sss^{\rm dl} \in \CC^{K \times 1}$ denote the vector of information bearing symbols for the $K$ users, assumed to 
%be zero mean, independent, with variance $q_k \geq 0$. 
%Under a general linear precoding scheme, we have
%\begin{equation} 
%	\xx = \UU \sss^{\rm dl}, \label{linear-precoding}
%\end{equation}
%where $\UU \in \CC^{LM \times K}$ is the overall precoding matrix, formed by $M \times 1$ blocks $\uv_{\ell,k}$ such that
%$\uv_{\ell,k} = \zerov$ if $(\ell, k) \notin \Ec$.  The non-zero blocks $\uv_{\ell,k} :  (\ell,k) \in \Ec$ contain the precoding vectors. Using (\ref{linear-precoding}) in (\ref{DLchannel}), we have
%\begin{eqnarray}
%	y^{\rm dl}_k & = & \hh_k^\herm \uu_k s^{\rm dl}_k   + \sum_{j \neq k} \hh_k^\herm \uu_j s^{\rm dl}_j  + z^{\rm dl}_k, 
%\end{eqnarray}
%where $\uu_k$ is the $k$-th column of $\UU$.  The resulting DL (optimistic) SINR, is given by 
%\begin{eqnarray}
%	\SINR^{\rm dl}_k & = & \frac{|\hh_k^\herm \uu_k|^2 q_k}{\SNR^{-1} + \sum_{j\neq k}   |\hh_k^\herm \uu_j|^2 q_j }, \label{DL-SINR} 
%\end{eqnarray}
%where $q_k$ is the DL transmit (Tx) power for UE $k$, such that the DL optimistic ergodic achievable rate is 
%\begin{equation}
%	R_k^{\rm dl} = \EE [ \log ( 1 + \SINR^{\rm dl}_k ) ]. \label{dl-ergodic-rate}
%\end{equation}
%
%Assuming that the columns of the precoder $\UU$ have unit norm, we have that the total DL Tx power collectively transmitted by the RRHs is given by 
%\begin{align} 
%	P^{\rm dl}_{\rm tot} &= \trace \left ( \EE [ \xx \xx^\herm ] \right ) = \trace \left ( \UU \diag(q_k : k \in [K]) \UU^\herm \right ) \\
%	&= \trace \left ( \UU^\herm \UU \diag(q_k : k \in [K]) \right ) = \sum_{k=1}^K q_k.  
%\end{align}
%We assume the UL and DL total transmit power to be balanced, which after scaling the LSFCs with the factor $\SNR$, imposes the condition $\sum_{k=1}^K q_k = K$. 


==> 03_channel_estimation.tex <==
%!TEX root = isit-paper.tex
\section{UL channel estimation}
In practice, ideal (although partial) CSI is not available and the channels $\{\hv_{\ell,k} : (\ell,k) \in \Ec\}$ must be estimated from
the UL DMRS pilots.  The DMRS pilot field received at RRH $\ell$ is given by the $M \times \tau_p$ matrix of received symbols
\begin{equation} 
\Ym_\ell^{\rm DMRS} = \sum_{i=1}^K \hv_{\ell,i} \phiv_{t_i}^\herm + \Zm_\ell^{\rm DMRS}, \label{Y_pilot} 
\end{equation}
where $\phiv_{t_i}$ denotes the DMRS pilot vector of dimension $\tau_p$ used by UE $i$ in the current RB, with  
total energy $\| \phiv_{t_i} \|^2 = \tau_p \SNR$.  For each UE $k \in \Uc_\ell$, RRH $\ell$ produces the {\em pilot matching} (PM) channel estimates
\begin{eqnarray} 
	\widehat{\hv}^{\rm pm}_{\ell,k} & = & \frac{1}{\tau_p \SNR} \Ym^{\rm DMRS}_\ell \phiv_{t_k}  \\
	& = & \hv_{\ell,k}  + \sum_{\substack{i : t_i = t_k \\ i\neq k}} \hv_{\ell,i}  + \widetilde{\zv}_{t_k,\ell} ,  \label{chest}
\end{eqnarray} 
where $\widetilde{\zv}_{t_k,\ell}$ has i.i.d. with components $\Cc\Nc(0, \frac{1}{\tau_p\SNR})$. 
Notice that the presence of UEs $i \neq k$ using the same DMRS pilot $t_k$ yields pilot contamination. 
%By the cluster construction rule, these users are not associated to any RRH in cluster $\Cc_k$ since pilot $t_k$ is ``occupied'' by UE $k$ 
%for all such RRHs.  

Assuming that the subspace information $\Fm_{\ell,k}$ of all $k \in \Uc_\ell$ is known, 
we consider also the {\em subspace projection} (SP)  pilot decontamination scheme for which the projected channel estimate is given by the 
orthogonal projection of $\widehat{\hv}^{\rm pm}_{\ell,k}$ onto the subspace spanned by the columns of $\Fm_{\ell,k}$, i.e., 
\begin{align}
	\widehat{\hv}^{\rm sp}_{\ell,k} &= \Fm_{\ell,k}\Fm_{\ell,k}^\herm \widehat{\hv}^{\rm pm}_{\ell,k} 
	%& = \hv_{\ell,k}  + \Fm_{\ell,k}\Fm_{\ell,k}^\herm \left ( \sum_{\substack{i : t_i = t_k \\ i\neq k}} \hv_{\ell,i} \right ) + \Fm_{\ell,k} \Fm_{\ell,k}^\herm \widetilde{\zv}_{t_k,\ell}  
	\label{chest1}
\end{align}
%Notice that after SP, the resulting estimation noise is correlated since it is contained in the channel subspace, 
%such that the covariance matrix of the projected noise is given by $\frac{1}{\tau_p\SNR} \Fm_{\ell,k} \Fm_{\ell,k}^\herm$. 
The pilot contamination term after the subspace projection  
%\begin{align}
%	\Fm_{\ell,k}\Fm_{\ell,k}^\herm \left ( \sum_{\substack{i : t_i = t_k \\ i\neq k}} \hv_{\ell,i} \right ) 
%	%&= \sum_{\substack{i : t_i = t_k \\ i\neq k}} \Fm_{\ell,k}\Fm_{\ell,k}^\herm \hv_{\ell,i} \nonumber  \\ 
%	& = \sum_{\substack{i : t_i = t_k \\ i\neq k}} \sqrt{\frac{\beta_{\ell,i} M}{|\Sc_{\ell,i}|}}  \Fm_{\ell,k}\Fm_{\ell,k}^\herm \Fm_{\ell,i} \nuv_{\ell,i} .
%\end{align}
is a Gaussian vector with mean zero and covariance matrix
\begin{equation}
	\Sigmam_{\ell,k}^{\rm co}  = \sum_{\substack{i : t_i = t_k \\ i\neq k}} \frac{\beta_{\ell,i} M}{|\Sc_{\ell,i}|}  \Fm_{\ell,k} \Fm_{\ell,k}^\herm \Fm_{\ell,i} \Fm^\herm_{\ell,i} \Fm_{\ell,k} \Fm^\herm_{\ell,k}. 
\end{equation}
When $\Fm_{\ell,k}$ and $\Fm_{\ell,i}$ are nearly mutually orthogonal, i.e. $\Fm_{\ell,k}^\herm \Fm_{\ell.i} \approx \zerov$,
the subspace projection is able to significantly reduce the DMRS pilot contamination effect.

==> 04_srs_pilots.tex <==
%!TEX root = isit-paper.tex
\section{Subspace estimation with UL SRS pilots}

In order to implement the DMRS channel estimation with pilot decontamination based on channel subspace projection in (\ref{chest1}), 
the dominant subspace of each user channel $\hv_{\ell,k}$ with $k \in \Uc_\ell$ must be estimated at each RU $\ell$. Such subspaces are long-term statistical properties 
that depend on the geometry of the propagation, which is assumed to remain essentially invariant over sequences of many consecutive slots, 
and it is frequency-independent. Furthermore, assuming ULAs or UPAs and owing to the Toeplitz or block-Toeplitz structure of the channel covariance matrices, 
for large $M$ such subspaces are nearly spanned by subsets of the DFT columns (see \cite{adhikary2013joint}). This also show that while our
one-ring scattering model may seem restrictive, it is actually general enough for large ULAs and UPAs, which is the most interesting 
and practical case for applications. 

In this section, we propose to use SRS pilots channel subspace estimation, where the sequence of SRS pilots spans a large number of slots and subcarriers in 
order to provide the necessary statistical averaging and capture the correct channel second-order statistics. We assume that each user sends just {\em one} SRS pilot symbol 
per slot, hopping over the subcarriers in multiple slots. In this sense, ``orthogonal SRS pilots'' indicate symbols send by different users on different subcarriers on the same slot. 
We reserve a grid of $N$ distinct subcarriers for the SRS pilot in each slot, such that in any slot time there exist 
$N$ orthogonal SRS pilots.  We say that two users have a SRS pilot collision at some slot, when they transmit their SRS pilot symbol on the same subcarrier. 
The allocation of SRS pilot sequences to users is done in order to minimize the pilot collisions between users at the RUs forming their clusters. 
It is clear that two users physically separated by a large distance can have pilot collisions without suffering from the mutual interference, since their corresponding clusters are also
physically separated. In contrast, it may happen that some user $k$ collides on some slot $s$ with some user $j$, and that user $j$ is much closer to  RU $\ell \in \Cc_k$ than user $k$. In this case, the measurement at RU $\ell$ relative to user $k$ is heavily interfered by such collision. 
Our scheme is based on a) allocating sequences such that such type of damaging collision is minimized, and b) using a subspace estimation method that is robust to 
a small number of heavily interfered measurements (outliers). This will be explained in details in the following. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Orthogonal latin squares-based SRS pilot hopping scheme} 
We employ an SRS pilot hopping scheme based on orthogonal latin squares \cite{467960}. 
A latin square of order $N$ is an $N \times N$ array $\Am$ with elements in $[N] = \{1,\ldots, N\}$ such that every row and column contain all distinct elements. 
Two latin squares $\Am$ and $\Bm$ are said to be mutually orthogonal if the collection of elementwise pairs 
$\{(\Am(i,j), \Bm(i,j)) : i,j \in [N]\}$ contains all $N^2$ distinct pairs. This means that the positions marked with $k \in [N]$ in $\Am$ are marked with all
possible distinct integers from 1 to $N$ in $\Bm$. 

\begin{example}  \label{latin-square}
	Consider $N = 5$ and the latin squares
	\begin{equation}
		\Resize{1.0\linewidth}{\Am = \begin{bmatrix}
			\boxed{1} & 2 & 3 & 4 & 5 \\
			2 & 3 & 4 & 5 & \boxed{1} \\
			3 & 4 & 5 & \boxed{1} & 2  \\
			4 & 5 & \boxed{1} & 2 & 3 \\
			5 & \boxed{1} & 2 & 3 & 4
		\end{bmatrix}  , \
		\Bm = \begin{bmatrix}
			\boxed{1} & 2 & 3 & 4 & 5  \\
			3 & 4 & 5 & 1 & \boxed{2} \\
			5 & 1 & 2 & \boxed{3} & 4  \\
			2 & 3 & \boxed{4} & 5 & 1  \\
			4 & \boxed{5} & 1 & 2 & 3 
		\end{bmatrix} . \nonumber}
	\end{equation}
	The positions marked by (say) 1 in $\Am$ (boxed positions) contain all elements $\{1,2,3,4,5\}$ in $\Bm$, and this holds for all symbols. hence, $\Am$ and $\Bm$ are orthogonal latin squares. \hfill $\lozenge$
\end{example}

The construction of families of $N - 1$ mutually orthogonal latin squares of order $N$ when $N$ is a prime power (i.e., $N = p^n$ for some prime $p$ and integer $n$) 
is well-known and given in \cite{467960}. In the proposed scheme, a latin square identifies $N$ hopping schemes as follows: we identify the rows of the 
latin square with the distinct subcarriers $f \in [N]$ used for SRS hopping (numbered from 1 to N without loss of generality) and 
the columns with the  time slots $s \in [N]$. 
Each latin square defines $N$ mutually orthogonal hopping sequences given by the sequence of positions $(f,s)$ corresponding to each integer $k \in [N]$. 
For example, in Example \ref{latin-square}, $N = 5$ users (say $k_1, k_2, \ldots, k_5$ are associated to the 5 mutually orthogonal hopping sequences
$\{ (f,s) : \Am(f,s) = n \}$, for $n = 1,2,\ldots, 5$ (e.g., user $k_1$ is associated to the sequence hopping over the boxed symbols in $\Am$ corresponding to index $n = 1$, and so on). 
If two users are associated to sequences in distinct orthogonal latin squares, they shall collide only in one hopping position. In other words, a user associated to latin square $\Am$ 
will collide on the $N$ hopping slots with each one of the $N$ users associated to the orthogonal latin square $\Bm$ (e.g., consider the boxed positions in $\Am$ and $\Bm$
in Example \ref{latin-square}, where user $k_1$ associated to $n = 1$ in $\Am$ collides with different users associated with hopping sequences $1, 5, 4, 3, 2$ 
in $\Bm$ (in the order of consecutive slots $s = 1,2,3,4,5$ indicating the columns of the latin square array). 
This creates a good averaging of interference. In particular, we partition the network coverage area into 
hexagonal cells, and allocate the $N-1$ latin squares in a classical reuse of order $N-1$, such that adjacent cells have distinct orthogonal latin squares. 
The hexagonal cells have nothing to do with the user-centric clusters and are defined on a purely geometric basis. In practice, one may consider that the cell-free user-centric network
co-exists on a different frequency band with an existing LTE or 5GNR cellular network, and that the latin square allocation is done based on the cells of the cellular network.
Since cell-free user-centric networks are often regarded as non-stand-alone networks to provide high data rates to users already operating in a conventional network through (possibly non-adjacent) carrier aggregation, and since 5G allows the decoupling of the control and data planes \cite{3gpp23501}, such allocation can be easily accomplished through the cellular network.  
As a consequence of this geographic reuse of the family of orthogonal latin squares, users in the same hexagonal cell have no mutual SRS pilot collisions, and users 
in adjacent cells have at most one mutual SRS pilot collision.  Hence,  if a user suffers from high interference from some other user in an adjacent cell, this will occur only in one out of $N$ 
SRS symbols. Notice that the good interference averaging property of orthogonal latin squares for slow hopping was already noticed in \cite{467960} 
in the context of 2G systems such as GSM. We conclude this section by saying that  in general the length of SRS hopping sequences $S$ may be larger than $N$. In this case, 
the time slot index $s$ is to be considered modulo $N$, that is, the sequence is periodically repeated. 


\subsection{Estimation via R-PCA}

Consider a generic RU $\ell$. The RU is aware of the SRS hopping sequence of all its associated users in $\Uc_\ell$. 
Focusing on some UE $k \in \Uc_\ell$, we describe now how the RU can estimate the channel subspace (column span of $\Fm_{\ell,k}$ in our simplified scattering model).
The RU collects all SRS pilot measurements corresponding to the hopping sequence of UE $k$. On slot $s \in [S]$ these are given by 
\begin{align}
	\yv_{\ell,k}^{\rm SRS}(s) 
	%& = & \frac{1}{ \SNR} \Ym^{\rm SRS}_\ell(s) \phiv_{t_k}^{\rm SRS}(s)  \\
	& =  \hv_{\ell,k} (s) + \sum_{i \neq k: t_i(s) = t_k(s) } \hv_{\ell,i} (s) + \widetilde{\zv}_{k,\ell}(s) \nonumber \\
	& =  \hv_{\ell,k} (s) + \sum_{\substack{i \neq k: \\ i \in \Ic^s_k(s) }} \hv_{\ell,i} (s) +  \sum_{\substack{i \neq k: \\ i \in \Ic^w_k(s) }} \hv_{\ell,i} (s) + \widetilde{\zv}_{k,\ell} (s) \nonumber \\
	& =  \hv_{\ell,k} (s) + \ev_{\ell,k} (s) +  \nv_{\ell,k} (s) ,
\end{align}
where $\widetilde{\zv}_{k,\ell}(s)$ is $M \times 1$ Gaussian i.i.d. with components $\Cc\Nc(0, \frac{1}{\SNR})$ and where the condition
$t_i(s) = t_k(s)$ indicate that the hopping sequence of user $i$ and of user $k$ collide at slot $s$ and where
the sets $\Ic^s_k(s)$ and $\Ic^w_k(s)$ contain the UEs colliding with UE $k$ with strong and weak LSFCs with respect to RU $\ell$, respectively. 
The term  $\ev_{\ell,k} (s) = \sum_{i \neq k: i \in \Ic^s_k(s) } \hv_{\ell,i} (s)$ accounts
accounts for the strong undesired signals (the so-called \textit{outliers}) while the term
$\nv_{\ell,k} = \sum_{i \neq k: i \in \Ic^w_k(s) } \hv_{\ell,i} (s) + \widetilde{\zv}_{k,\ell} (s)$ includes noise and weak interference.
Stacking the $S$ SRS pilot observations as columns of a $M \times S$ array, we have
\begin{eqnarray}
	\Ym^{\rm SRS}_{\ell,k} & = & [\yv_{\ell,k}^{\rm SRS}(1) \ \yv_{\ell,k}^{\rm SRS}(2) \dots \yv_{\ell,k}^{\rm SRS}(S)] \label{Y_concat} \\
	& = & \Hm_{\ell,k} + \Nm_{\ell,k} + \Em_{\ell,k}, 
\end{eqnarray}
where $\Hm_{\ell,k}$, $\Nm_{\ell,k}$ and $\Em_{\ell,k}$ are given by the analogous stacking of vectors $\hv_{\ell,k} (s), \ev_{\ell,k} (s)$ and $ \nv_{\ell,k} (s)$, respectively. 
Because of the orthogonal latin squares hopping patterns, it is expected that 
$\Em_{\ell,k}$ is column-sparse to a certain degree.  This is equivalent to the noise plus outliers model in \cite{6126034}. 
The R-PCA algorithm in  \cite{6126034} aims at detecting outliers the non-zero columns of $\Em_{\ell,k}$ and at estimating the subspace of $\Hm_{\ell,k}$, which eventually is the desired channel subspace
of UE $k$ at RU $\ell$. Fixing some appropriate $\epsilon > 0$ such that  $\lVert \Nm_{\ell,k} \rVert_F \leq \epsilon$ with high probability, and $\lambda > 0$, 
the algorithm solves the  convex problem
\begin{eqnarray}
	\underset{ \Hm_{\ell,k}, \Em_{\ell,k} }{\text{minimize}} & & \lVert \Hm_{\ell,k} \rVert_* + \lambda \lVert \Em_{\ell,k} \rVert_{2,1} \label{pca_opt_problem} \\
	\text{subject to:} & & \lVert \Ym^{\rm SRS}_{\ell,k} - \Hm_{\ell,k} - \Em_{\ell,k} \rVert_F \leq \epsilon, \nonumber
\end{eqnarray}
where $\lVert \cdot \rVert_*$, $\lVert \cdot \rVert_F$, and $\lVert \cdot \rVert_{2,1}$ denote the nuclear norm, the Frobenius norm, and the sum of the $\ell_2$ column norms of a matrix, respectively. The Lagrangian function of (\ref{pca_opt_problem}) is given by 
\begin{align}
	\Lc &\left (\Hm_{\ell,k}, \Em_{\ell,k}, \lambda, \mu \right )   = \lVert \Hm_{\ell,k} \rVert_* \nonumber \\  &+ \lambda \lVert \Em_{\ell,k} \rVert_{2,1} + \mu \left ( \lVert \Ym^{\rm SRS}_{\ell,k} - \Hm_{\ell,k} - \Em_{\ell,k} \rVert_F - \epsilon \right ),
\end{align}
where $\mu$ is a Lagrange multiplier.
Therefore, the corresponding unconstrained convex minimization problem is given as
\begin{align}
	\underset{ \Hm_{\ell,k}, \Em_{\ell,k} }{\min}  \; \underset{\mu \geq 0}{\max} \hspace{.2cm} \Lc \left (\Hm_{\ell,k}, \Em_{\ell,k}, \lambda, \mu \right ). \label{pca_convex}
\end{align}
We employ the algorithm proposed in \cite{6126034} to approach (\ref{pca_convex}), which returns estimates $\widehat{\Hm}_{\ell,k}$ and $\widehat{\Em}_{\ell,k}$ 
of the channel and outliers matrix, respectively. 
The parameter $\lambda$ is given as an input to the algorithm and is optimized empirically. If the rank of the resulting $\widehat{\Hm}_{\ell,k}$ is larger (smaller) than expected, we decrease (increase) $\lambda$. The algorithm does not require $\epsilon$ to be specified and treats the observation matrix as in the noiseless case. Note that $\epsilon$ however is important for the analytical results of the algorithm in \cite{6126034}. The Lagrange multiplier $\mu$ is optimized by the algorithm via primal-dual iterations.



From the SVD $\widehat{\Hm}_{\ell,k} = \widehat{\Um}\widehat{\Sm} \widehat{\Vm}^\text{H}$, we estimate the subspace by considering the left singular vectors (columns of $\widehat{\Um}$ corresponding to the dominant singular values. One approach to find the number of dominant singular values is to find the index at which there is the largest difference (gap) between consecutive singular values.

%\begin{figure}[t]
%	\centerline{\includegraphics[trim={0 0 0 1.1cm},clip,width=8cm]{results/sing_values_separation}}
%	\caption{Example for the normalized singular values of a channel matrix estimate of the R-PCA subspace estimate, where $M=32$. In this case, we have $r^{\rm PCA} = 4$ dominant singular values, as the gap between the 4th and 5th singular value is the largest difference between consecutive singular values.}
%	\label{sing_values_separation}
%\end{figure}

%Having $r^{\rm PCA}$ dominant singular values, the subspace estimate is given by 
%\begin{eqnarray}
%	\widehat{\Fm}_{\ell,k}^{\rm PCA} = \widehat{\Um}_{:,1:r^{\rm PCA}}
%\end{eqnarray}
%and the estimated covariance matrix by
%\begin{eqnarray}
%	\Sigma_\hv \left(\widehat{\Fm}_{\ell,k}^{\rm PCA}\right) = \frac{\beta_{\ell,k}M}{r^{\rm PCA}} \widehat{\Fm}_{\ell,k}^{\rm PCA}\left(\widehat{\Fm}_{\ell,k}^{\rm PCA}\right)^\text{H}.
%\end{eqnarray}
Let $\widehat{\Fm}_{k,\ell}^{\rm PCA} = \widehat{\Um}_{:,1:r^{\rm PCA}}$ denote the tall unitary matrix obtained by selecting the dominant $r^{\rm PCA}$ left eigenvectors as explained above.  We can further post-process the subspace estimate by imposing that its basis vectors are DFT columns. 
As anticipated before, this is motivated by the fact that, for large Toeplitz matrices, the eigenvectors are closely approximated by DFT vectors \cite{adhikary2013joint}. 
The identification of the best fitting DFT columns to the R-PCA estimated subspace can be done greedily by finding one by one the $r^{\rm PCA}$ columns $\Fm_{:,i}$ of $\Fm$ 
that maximize the quantity
\begin{eqnarray}
	\Fm_{:,i}^\herm \widehat{\Fm}_{k,\ell}^{\rm PCA} (\widehat{\Fm}_{k,\ell}^{\rm PCA})^\herm \Fm_{:,i}.
\end{eqnarray}
We denote the selected set of column indices as $\widehat{\Sc}_{\ell,k}^{\rm PP}$, such that the corresponding estimated projected PCA (PP) 
subspace is given by $\widehat{\Fm}_{\ell,k}^{\rm PP} = \Fm(: , \widehat{\Sc}_{\ell,k}^{\rm PP})$. The estimated channel covariance matrix for a given subspace estimate 
$\widehat{\Fm}_{k,\ell}$ is given by 
\begin{eqnarray}
	\Sigma_{\hv}(\widehat{\Fm}_{\ell,k}) = \frac{\beta_{\ell,k} M}{r^{\rm PCA}} \widehat{\Fm}_{\ell,k} \widehat{\Fm}_{\ell,k}^\herm, 
\end{eqnarray} 
where $\widehat{\Fm}_{k,\ell} = \widehat{\Fm}_{k,\ell}^{\rm PCA}$ or $\widehat{\Fm}_{k,\ell} = \widehat{\Fm}_{k,\ell}^{\rm PP}$, depending on the considered case. 

In order to evaluate the quality of a generic subspace estimate $\widehat{\Fm}_{\ell,k}$, we consider the power efficiency defined by 
\begin{eqnarray}
	E_{\rm PE}(\widehat{\Fm}_{\ell,k}) = \frac{\trace\left(\Sigma_{\hv}(\Fm_{\ell,k}) \Sigma_{\hv}(\widehat{\Fm}_{\ell,k}) \right)}{\trace\left(\Sigma_{\hv}(\Fm_{\ell,k}) \Sigma_{\hv}(\Fm_{\ell,k}) \right)},
\end{eqnarray}
%where $\Sigma_{\hv}(\Fm_{\ell,k}) = \frac{\beta_{\ell,k} M}{|\Sc_{\ell,k}|} \Fm_{\ell,k} (\Fm_{\ell,k})^\herm$. 
The power efficiency $E_{\rm PE}(\widehat{\Fm}_{\ell,k}) \in [0,1]$ measures how much power from the desired channel in (\ref{chest1}) is captured in the channel estimate. 
%Additionally, we consider also the normalized Frobenius-norm error given by
%\begin{eqnarray}
%	E_{\rm NF}(\widehat{\Fm}_{\ell,k}) = \frac{ \lVert \Sigma_{\hv}(\Fm_{\ell,k}) - \Sigma_{\hv}(\widehat{\Fm}_{\ell,k}) \rVert_\text{F} }{\lVert \Sigma_{\hv}(\Fm_{\ell,k}) \rVert_\text{F}}.
%\end{eqnarray}

==> 05_simulations.tex <==
%!TEX root = isit-paper.tex
\section{Simulations and concluding remarks} \label{sec:ul_perfect_csi}
In our simulations, we consider a square coverage area of $A = 225 \times 225$ square meters with a torus topology to avoid boundary effects. 
The LSFCs are given  according to the 3GPP urban microcell pathloss model from \cite{3gpp38901}. 
The parameter $\SNR$ is chosen such that $\bar{\beta} M \SNR = 1$ (i.e., 0 dB), when the expected pathloss $\bar{\beta}$ with respect to LOS and NLOS is calculated for distance $3 d_L$, where $d_L = 2 \sqrt{\frac{A}{\pi L}}$ is the diameter of a disk of area equal to $A/L$.
We consider RBs of dimension $T = 200$ symbols. 
{\RED The UL (same for DL) spectral efficiency (SE) for UE $k$ is given by  ${\rm SE}^{\rm ul}_k =  (1 - \taudmrs/T) R_k^{\rm ul}$. (AT THE MOMENT ONLY UPLINK AND DATA RATES ARE SHOWN.)}
The angular support $\Sc_{\ell,k}$ contains the DFT quantized angles (multiples of $2\pi/M$) falling inside an interval of length $\Delta$ placed symmetrically around the direction joining UE $k$ and RRH $\ell$. We use $\Delta = \pi/8$ and the maximum cluster size $Q=10$ (RRHs serving one UE) in the simulations. The SNR threshold $\eta=1$ makes sure that an RRH-UE association can only be established, when $\beta_{\ell,k} \geq \frac{\eta}{M \SNR } $. \textcolor{red}{We consider two systems, where the first contains $L=10$ RRHs with $M=64$ antennas, $K=100$ UEs and we use $\taudmrs = 40$, while for the second $L=20$, $M=32$, $K=100$ and $\taudmrs = 20$. These choices of $\taudmrs$ lead to a good system performance with diffferent UL combining and DL precoding schemes \cite{kddi_uldl_precoding}.}

\begin{figure}[t!]
	\centerline{\includegraphics[width=4.4cm]{figures/cdf_comp_srs_K100_L10_M64_dmrs040_eta1_q10_delta0p392699_samples200_lambda0p40_setups300}  \hspace{-.1cm}
	\includegraphics[width=4.4cm]{figures/cdf_comp_srs_K100_L20_M32_dmrs020_eta1_q10_delta0p392699_samples200_lambda0p30_setups300}}
	\caption{The power efficiency of the R-PCA subspace estimates with $L=10, M=64$ (left) and $L=20, M=32$ (right).}
	\label{subspace_estimation_results_pca}
\end{figure}
Figure \ref{subspace_estimation_results_pca} shows the empirical cdf of the PE of the subspace estimates for $N=\{19, 61\}$ in the two systems, where the cdfs are computed from the subspace estimates of all associated RRH-UE pairs in 300 different layouts (random uniform placement of RRHs and UEs). The impact of $N$ is clear, as the SRS pilot hopping with $N=61$ yields a much larger fraction of estimates with large energy efficiency compared to $N=19$. Due to the projection of the estimates onto the columns of the DFT matrix, the PE of the ``Projected R-PCA" estimates follows a discrete distribution, which follows approximately the continuous distribution of the ``R-PCA" estimates before projection. The fraction of estimates with high PE is increased for $L=20$ compared to $L=10$, since the R-PCA performance is highly dependent on the SNR of the UL SRS pilot signal (see Fig. \ref{compare_rpca_pdf_vs_beta_ranges} {\RED Do we need this figure? It consumes a lot of space and it should be expected that higher SNR leads to better estimates.}), and the RRH-UE association becomes more selective due to the smaller $\taudmrs$ for $L=20$. 

\begin{figure}[t]
	\centerline{\includegraphics[width=7.8cm]{figures/isit_cdf_pe_snr_ranges_K100_L10_M64_dmrs040_srs061_eta1_q10_delta0p392699_samples200_lambda0p40_setups300} }
	\caption{The power efficiency with the R-PCA algorithm in different channel gain ranges, where $L=10$, $M=64$, $\taudmrs=40$ and $N = 61$. Low SNR accounts for the dataset of the channel gains in the 5th percentile, medium SNR for the channel gains between the 10th and 15th percentile, high SNR for the channel gains above the 30th percentile. The whole dataset contains the samples from the 300 topologies evaluated in Fig. \ref{subspace_estimation_results_pca}.}
	\label{compare_rpca_pdf_vs_beta_ranges}
\end{figure}

\subsection{System performance with subspace estimates}
\begin{figure}[t!]
	\centerline{\includegraphics[width=4.4cm, trim={.3cm .1cm 1.5cm .9cm}, clip]{figures/isit_rate_ul_K100_L10_M64_tau_p_dmrs040_tau_srs019_eta1_q10_setups100}  \hspace{-.1cm}
	\includegraphics[width=4.4cm, trim={.3cm .1cm 1.5cm .9cm}, clip]{figures/isit_rate_ul_K100_L10_M64_tau_p_dmrs040_tau_srs061_eta1_q10_setups100}}
	\centerline{\includegraphics[width=4.4cm, trim={.3cm .1cm 1.5cm .9cm}, clip]{figures/isit_rate_ul_K100_L20_M32_tau_p_dmrs020_tau_srs019_eta1_q10_setups100}  \hspace{-.1cm}
	\includegraphics[width=4.4cm, trim={.3cm .1cm 1.5cm .9cm}, clip]{figures/isit_rate_ul_K100_L20_M32_tau_p_dmrs020_tau_srs061_eta1_q10_setups100}}
	\caption{The UL data rates for $L=10$, $M=64$ (top row) and $L=20$, $M=32$ (lower row). From left to right $N = \{19, 61\}$.}
	\label{rate_evaluation_pca}
\end{figure}
We evaluate the \textcolor{red}{UL (should we add DL results? Could get tight with 5 pages limit + extra page for references)} optimistic ergodic achievable rates in a cell-free network, where we compare the performance using subspace estimates for subspace projection channel estimation in (\ref{chest1}) to the cases of ideal partial CSI, and channel estimation with pilot matching in (\ref{chest}) and perfect subspace knowledge in (\ref{chest1}), respectively.
For each set of parameters we generated 100 independent layouts, 
and for each  layout we computed the expectation in (\ref{ergodic-rate}) 
%and (\ref{dl-ergodic-rate}) 
by Monte Carlo averaging with respect to the channel vectors. 
In the UL, we employ RRH cluster wise global zero-forcing (GZF) combining, as well as local linear MMSE (LMMSE) with global combining. 
%In the DL, we use GZF precoding, local LMMSE with centralized power allocation, and local ZF (LZF) with local proportional power allocation to the LSFCs. 
We refer to \cite{kddi_uldl_precoding} for details of the schemes. 
Figure \ref{rate_evaluation_pca} shows that the gap between the rates with perfect subspace knowledge (denoted by ``SP") and subspace estimates (``R-PCA-SP") can be basically closed, when using a sufficiently large number of UL SRS pilots. In that case, even the rates with ideal partial CSI (``full CSI") can be closely approached, while the system performance using PM is limited due to pilot contamination. 
%Note that for $L=20$, $M=32$ we use $\taudmrs= 20$, which optimizes the system performance \textcolor{red}{(see [WCNC paper])} and leads to better subspace estimates compared to the system with $L=10$ and $\taudmrs= 40$.
Having $N = 19$ in the system with $L=10$, PM and R-PCA-SP yield similar rates, while no difference between subspace projection with perfect subspace knowledge and estimates is visible for $L=20$ and $N = 61$. In the other two cases, a small degradation of the rates is observed when replacing the true subspace with the estimate from the R-PCA algorithm.

The results show that the proposed SRS pilot assignment and subspace estimation schemes under practical assumptions can basically obtain the same performance as a system with perfect subspace information. Furthermore, channel estimation using subspace estimates yields data rates which approach very closely the performance of perfect CSI, pointing out the powerfulness of subspace information, especially under the aspect that subspace knowledge is less challenging to obtain than the covariance matrix.



